WorldCoder, a Model-Based LLM Agent: Building World Models by Writing Code and Interacting with the Environment

We give a model-based agent that builds a Python program representing its knowledge of the world based on its interactions with the environment. The world model tries to explain its interactions, while also being optimistic about what reward it can achieve. We define this optimism as a logical constraint between a program and a planner. We study our agent on gridworlds, and on task planning, finding our approach is more sample-efficient compared to deep RL, more compute-efficient compared to ReAct-style agents, and that it can transfer its knowledge across environments by editing its code.

==> trajecotires/curri-plan-s1/fig.tex <==
Too long, do it later....

\begin{tcbitemize}[raster columns=3, raster equal height=rows,
size=small,]

\tcbitem[colback=white,colframe=white]

\tcbitem[title=Original reward function,colback=white]
\begin{lstlisting}[style=python]
NULL
\end{lstlisting}


\tcbitem[title=Original transit function,colback=white]
\begin{lstlisting}[style=python]
NULL
\end{lstlisting}


\tcbitem[title={Random exploration\\~},colback=white]
\includegraphics[width=\textwidth]{trajecotires/curri-plan-s1/env0-step0-12.png}


\tcbitem[title={Data-consistent transit-func\\
(figured out rotation and move forward)},colback=white, raster multicolumn=2, colframe=yellow!50!black]
\begin{lstlisting}[style=python]
def rotate_right(direction):
    if direction == (0, 1):
        return (-1, 0)
    elif direction == (1, 0):
    ...
def rotate_left(direction):
    if direction == (0, 1):
        return (1, 0)
    elif direction == (1, 0):
    ...
def move_forward(agent, next_state):
    dx, dy = agent.direction
    new_x, new_y = agent.x + dx, agent.y + dy
    entities_in_cell = get_entities_by_position(next_state, new_x, new_y)
    if any(entity.name in {"Wall", "Box"} for entity in entities_in_cell): # non-moveable entities
        return False
    # checking boundaries of `x` and `y`
    x_values = [entity.x for entity in next_state]
    y_values = [entity.y for entity in next_state]
    if not (min(x_values) <= new_x <= max(x_values) and min(y_values) <= new_y <= max(y_values)):
        return False
    agent.x, agent.y = new_x, new_y
    return True
def transition(state, action):
    next_state = set(entity for entity in state)
    agent = get_entities_by_name(state, 'Agent')[0]
    next_state.remove(agent)
    if action == "turn right":
        agent.direction = rotate_right(agent.direction)
    elif action == "turn left":
        agent.direction = rotate_left(agent.direction)
    elif action == "move forward":
        moved = move_forward(agent, next_state)
        if not moved:
            next_state.add(agent)
            return next_state
    # handle other actions as before 
    # add the agent back to the state
    next_state.add(agent)
    return next_state
\end{lstlisting}

\tcbitem[colback=white,colframe=white]

\tcbitem[title={Data-consistent reward-func\\
(synthesized given the textual mission. Failed to generate positive rewards. Non-compatible with the input format either.)},colback=white, raster multicolumn=2, colframe=yellow!50!black]
\begin{lstlisting}[style=python]
def reward_func(state, action, next_state):
    # (*@\codehlerr{the reward is always 0.0 regardless of the action}@*)
    reward = 0.0
    # extract the agent from the next_state
    next_agent = get_entities_by_name(next_state, 'Agent')[0]
    # get the position of the goal
    (*@\codehlerr{goal\_pos = [(entity.x, entity.y) for entity in next\_state if isinstance(entity, Goal)][0]}@*)
    # Check if the agent's next position is at the goal
    done = (next_agent.x, next_agent.y) == goal_pos
    return reward, done
\end{lstlisting}

\tcbitem[colback=white,colframe=white]

\tcbitem[title={Goal-driven reward-func\\
(found the almost correct reward-func with no more interaction)},colback=white, raster multicolumn=2, colframe=green!50!black]
\begin{lstlisting}[style=python]
def reward_func(state, action, next_state):
    reward = 0.0  # initialise reward as 0.0 for all actions
    # extract the agent from the current and next state
    agent = get_entities_by_name(state, 'Agent')[0]
    next_agent = get_entities_by_name(next_state, 'Agent')[0]
    # if the agent reaches the goal in the next state, the reward is 1.0 and the episode is done
    if (*@\codehlerr{len(get\_entities\_by\_position(state, next\_agent.x, next\_agent.y)) > 1}@*):
        done = True
        (*@\codehlerr{reward = 1.0}@*)
    else:
        done = False
    return reward, done

\end{lstlisting}

\tcbitem[title={Guided by corrected reward-func\\Find the goal and the positive reward},colback=white]
\includegraphics[width=\textwidth]{trajecotires/curri-plan-s1/env0-step16-18.png}


\tcbitem[title={Data-consistent reward-func\\
(found the correct reward-func)},colback=white, raster multicolumn=2, colframe=red!50!black]
\begin{lstlisting}[style=python]
def reward_func(state, action, next_state):
    reward = 0.0  
    done = False ns
    ## extract the agent from the current and next state
    agent = get_entities_by_name(state, 'Agent')[0]
    next_agent = get_entities_by_name(next_state, 'Agent')[0]
    ## If the agent reaches the goal in the next state, the reward is 1.0 and the episode is done
    agent_position_entities = get_entities_by_position((*@\codehlerr{next\_state}@*), next_agent.x, next_agent.y)
    for entity in agent_position_entities:
        if isinstance(entity, Goal):
            done = True
            reward = 1.0
            break
    return reward, done

\end{lstlisting}

\tcbitem[title={Solved MiniGrid-Empty\\Enter MiniGrid-DoorKey\\Trying to cross a locked door},colback=white]
\includegraphics[width=\textwidth]{trajecotires/curri-plan-s1/env11-step0-1.png}





\end{tcbitemize}










\begin{figure}[h!]
\begin{tcbitemize}[raster columns=2, raster equal height=rows,
size=small]
\tcbitem[title=C++,colback=white]\begin{lstlisting}[style=cpp]
int remainder_7_large_numbers ( string num ) {
  int series [ ] = {
    1, 3, 2, - 1, - 3, - 2 };
    int series_index = 0;
    int result = 0;
    for ( int i = num . size ( ) - 1; i >= 0; i -- ) {
      (*@\codehl{int digit = num [ i ] - '0';}@*)
      result += digit * series [ series_index ];
      series_index = ( series_index + 1 ) % 6;
      result %= 7;
    }
    if ( result < 0 ) result = ( result + 7 ) % 7;
    return result;
  }
\end{lstlisting}
\tcbitem[title=Original Python,colback=white]
\begin{lstlisting}[style=python]
def remainder_7_large_numbers(num):
    series = [1, 3, 2, -1, -3, -2]
    series_index = 0
    result = 0
    for i in range((len(num) - 1), -1, -1):
        (*@\codehl{digit = (num[i] - '0')}@*)
        result += (digit * series[series_index])
        series_index = ((series_index + 1) % 6)
        result %= 7
    if (result < 0):
        result = ((result + 7) % 7)
    return result
\end{lstlisting}
\end{tcbitemize}
\begin{tcolorbox}[title=Self-debugging with UT feedback, left=2mm,right=1mm,top=0.5mm,bottom=0mm, colback=white,colframe=green!50!black]
\begin{lstlisting}[style=text]
The Python translation does not do the same thing as the C++ code. These are the results of one failed unit test that tests whether the Python translation's outputs match the C++ program's outputs:
Failed: assert remainder_7_large_numbers('K') == 6
Actual Result: Python runtime error: Traceback (most recent call last):
  File <filename>, line 29, in <module>
    print(remainder_7_large_numbers('K') )
  File <filename>, line 22, in remainder_7_large_numbers
    digit = (num[i] - '0')
TypeError: unsupported operand type(s) for -: 'str' and 'str'
Correct the Python translation.
\end{lstlisting}
\tcblower
\begin{lstlisting}[style=python]
def remainder_7_large_numbers(num):
    series = [1, 3, 2, -1, -3, -2]
    series_index = 0
    result = 0
    for i in range((len(num) - 1), -1, -1):
        (*@\codehl{digit = (ord(num[i]) - ord('0'))}@*)
        result += (digit * series[series_index])
        series_index = ((series_index + 1) % 6)
        result %= 7
    if (result < 0):
        result = ((result + 7) % 7)
    return result
\end{lstlisting}
\end{tcolorbox}
\caption{An example where \ours{} with unit test feedback fixes the code translation error, while the simple feedback fails.}
\label{fig:transcoder-ut-better-ex-1}
\end{figure}
